Sparsity-based audio declipping methods: selected overview, new algorithms, and large-scale evaluation

Recent advances in audio declipping have substantially improved the state of the art.% in certain saturation regimes. Yet, practitioners need guidelines to choose a method, and while existing benchmarks have been instrumental in advancing the field, larger-scale experiments are needed to guide such choices. First, we show that the clipping levels in existing small-scale benchmarks are moderate and call for benchmarks with more perceptually significant clipping levels. We then propose a general algorithmic framework for declipping that covers existing and new combinations of variants of state-of-the-art techniques exploiting time-frequency sparsity: synthesis vs. analysis sparsity, with plain or structured sparsity. Finally, we systematically compare these combinations and a selection of state-of-the-art methods. Using a large-scale numerical benchmark and a smaller scale formal listening test, we provide guidelines for various clipping levels, both for speech and various musical genres. The code is made publicly available for the purpose of reproducible research and benchmarking.

==> figures/others/CosparseDiagram.tex <==
	

	

	

	
	%% read the file
	\pgfplotstableread{AnalysisOperator.cvs}{\Analysisfile}
	\pgfplotstableread{TimeVect.cvs}{\TimeVectfile}
	\pgfplotstableread{SparseVect.cvs}{\SparseVectfile}
		
		\def\szx{7pt}
		\def\szy{7pt}
		
	
		\begin{equation}
		\label{eq:SparseAnalysis}
		\begin{array}{c c c c c}
		\begin{tikzpicture}[baseline={([yshift=-\szy]current bounding box.center)}]
		\pgfplotstableforeachcolumn\SparseVectfile\as\col{
			\pgfplotstableforeachcolumnelement{\col}\of\SparseVectfile\as\colcnt{%
				\draw[draw=blue,very thin,fill=red!\colcnt]($ -\pgfplotstablerow*(0,\szy) + \col*(\szx,0) $) rectangle+(\szx,\szy); 
			}
		}
		\end{tikzpicture} & = &
		\begin{tikzpicture}[baseline={([yshift=-\szy]current bounding box.center)}]
		\pgfplotstableforeachcolumn\Analysisfile\as\col{
			\pgfplotstableforeachcolumnelement{\col}\of\Analysisfile\as\colcnt{%
				\draw[draw=blue,very thin,fill=red!\colcnt]($ -\pgfplotstablerow*(0,\szy) + \col*(\szx,0) $) rectangle+(\szx,\szy); 
			}
		}
		\end{tikzpicture} & 
		\times  &
		\begin{tikzpicture}[baseline={([yshift=-\szy]current bounding box.center)}]
		
		\pgfplotstableforeachcolumn\TimeVectfile\as\col{
			\pgfplotstableforeachcolumnelement{\col}\of\TimeVectfile\as\colcnt{%
				\draw[draw=blue,very thin,fill=red!\colcnt]($ -\pgfplotstablerow*(0,\szy) + \col*(\szx,0) $) rectangle+(\szx,\szy); 
			}
		}	
		\end{tikzpicture}\\
		\vect{z} &  & \mtrx{A}  &  & \vect{x}
		\end{array}
		\end{equation}

		
		

==> figures/others/SparseDiagram.tex <==
	

	

	

	
	%% read the file
	\pgfplotstableread{Dictionary.cvs}{\Dictionaryfile}
	\pgfplotstableread{TimeVect.cvs}{\TimeVectfile}
	\pgfplotstableread{SparseVect.cvs}{\SparseVectfile}
		
		\def\szx{7pt}
		\def\szy{7pt}
		
	
		\begin{equation}
		\label{eq:SparseSynthesis}
		\begin{array}{c c c c c}
		\begin{tikzpicture}[baseline={([yshift=-\szy]current bounding box.center)}]
		
		\pgfplotstableforeachcolumn\TimeVectfile\as\col{
			\pgfplotstableforeachcolumnelement{\col}\of\TimeVectfile\as\colcnt{%
				\draw[draw=blue,very thin,fill=red!\colcnt]($ -\pgfplotstablerow*(0,\szy) + \col*(\szx,0) $) rectangle+(\szx,\szy); 
			}
		}	
		\end{tikzpicture} &
		= &
		\begin{tikzpicture}[baseline={([yshift=-\szy]current bounding box.center)}]
		
		\pgfplotstableforeachcolumn\Dictionaryfile\as\col{
						\pgfplotstableforeachcolumnelement{\col}\of\Dictionaryfile\as\colcnt{%
							\draw[draw=blue,very thin,fill=red!\colcnt]($ -\pgfplotstablerow*(0,\szy) + \col*(\szx,0) $) rectangle+(\szx,\szy); 
						}
					}
		\end{tikzpicture} &
		\times &
		\begin{tikzpicture}[baseline={([yshift=-\szy]current bounding box.center)}]
		
						\pgfplotstableforeachcolumn\SparseVectfile\as\col{
					\pgfplotstableforeachcolumnelement{\col}\of\SparseVectfile\as\colcnt{%
						\draw[draw=blue,very thin,fill=red!\colcnt]($ -\pgfplotstablerow*(0,\szy) + \col*(\szx,0) $) rectangle+(\szx,\szy); 
					}
				}
		\end{tikzpicture} \\
		\vect{x} &  & \mtrx{D} &  & \vect{z}
		\end{array}
		\end{equation}
		
